Towards a Workload for Evolutionary Analytics

Emerging data analysis involves the ingestion and exploration of new data sets, application of complex functions, and frequent query revisions based on observing prior query answers. We call this new type of analysis evolutionary analytics and identify its properties. This type of analysis is not well represented by current benchmark workloads. In this paper, we present a workload and identify several metrics to test system support for evolutionary analytics. Along with our metrics, we present methodologies for running the workload that capture this analytical scenario.

==> Makefile <==
SHELL := /bin/bash
TEXFORMATS := ".:styles/:" 
TEXINPUTS  := ".:pics/:styles/:"
BSTINPUTS  := ".:pics/:styles/:"
# SRC = viewfinder-single
SRC = benchmark

compile:
	export TEXFORMATS=${TEXFORMATS};  \
	export TEXINPUTS=${TEXINPUTS};  \
	export BSTINPUTS=${BSTINPUTS};  \
	bibtex ${SRC};  \
	pdflatex ${SRC}; 


==> conclusion.tex <==
\section{conclusion and Future work}\label{sec-conclusion}

We presented a query workload as a first-step ...

Future work to extend and improve the queries ...

\begin{comment}
Queries can be extended and refactored to incorporate additional
 data sources such as census data, geographical data, or historical business 
 data.

Queries may incorporate more diverse ML operations such as NLP, 
different classifiers, predictors, or recommender algorithms as UDFs.

UDFs could be implemented in a common language, say Java, or one of the 
languages a data management system supports.
Another option is to support UDF calls to different tools directly, 
\textit{i.e.}, Matlab or SAS, thus showcasing a system's flexibility for 
incorporating other non-native data analysis tools or functionality.
\end{comment}

